Geographic Gossip: Efficient Averaging for Sensor Networks

Gossip algorithms for distributed computation are attractive due to their simplicity, distributed nature, and robustness in noisy and uncertain environments. However, using standard gossip algorithms can lead to a significant waste in energy by repeatedly recirculating redundant information. For realistic sensor network model topologies like grids and random geometric graphs, the inefficiency of gossip schemes is related to the slow mixing times of random walks on the communication graph. We propose and analyze an alternative gossiping scheme that exploits geographic information. By utilizing geographic routing combined with a simple resampling method, we demonstrate substantial gains over previously proposed gossip protocols. For regular graphs such as the ring or grid, our algorithm improves standard gossip by factors of $n$ and $\sqrt{n}$ respectively. For the more challenging case of random geometric graphs, our algorithm computes the true average to accuracy $\epsilon$ using $O(\frac{n^{1.5}}{\sqrt{\log n}} \log \epsilon^{-1})$ radio transmissions, which yields a $\sqrt{\frac{n}{\log n}}$ factor improvement over standard gossip algorithms. We illustrate these theoretical results with experimental comparisons between our algorithm and standard methods as applied to various classes of random fields.

==> GossipMacros-1.tex <==
%% Theorem environments, etc
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}


%% shortcuts for environments
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\stexp}{\mbox{$\mathsf{E}$}}    % Statistical Expectation operator
\newcommand{\var}{\mbox{$\mathsf{Var}$}}    % Statistical variance
\def\qed{\quad \vrule height6.5pt width6pt depth0pt} %Nifty end proof sign
\newcommand{\bigO}{\mbox{$\mathsf{O}$}}  %Nifty bigO symbol

\newcommand{\EE}{ \mathcal{E}} %Nifty Energy symbol


%% shortcuts for mathmode
\def\tr{\mathop{\rm tr}\nolimits}       % tr for trace
\def\mbf{\mathbf}
\def\argmin{\mathop{\rm argmin}}
\newcommand{\diag}{\ensuremath{\operatorname{diag}}}
\def\mc{\mathcal}
\newcommand{\X} {\mathcal{X}}



%% misc other macros
\long\def\symbolfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}



%% macros for variables, etc
\newcommand{\Wmat}{\ensuremath{W}}
\newcommand{\Pmat}{\ensuremath{P}}
\newcommand{\ones}{\ensuremath{\vec{1}}}
\newcommand{\defn}{\ensuremath{: \, = }}
\newcommand{\avec}{\ensuremath{\vec{a}}}
\newcommand{\bvec}{\ensuremath{\vec{b}}}
\newcommand{\qvec}{\ensuremath{\vec{q}}}
\newcommand{\yvec}{\ensuremath{\vec{y}}}
\newcommand{\eigtwo}{\ensuremath{\lambda_2}}
\newcommand{\eigmax}{\ensuremath{\lambda_{\operatorname{max}}}}
\newcommand{\order}{\ensuremath{\mathcal{O}}}
\newcommand{\rejeps}{\ensuremath{\mu}}
\newcommand{\rejdelta}{\ensuremath{\nu}}
\newcommand{\Prob}{\ensuremath{\mathbb{P}}}
\newcommand{\dur}{\ensuremath{\mathcal{D}}}
\newcommand{\Qnum}{\ensuremath{Q}}
\newcommand{\Exs}{\ensuremath{\mathbb{E}}}
\newcommand{\xave}{\ensuremath{\bar{x}_{\operatorname{ave}}}}
%\newcommand{\ones}{\ensuremath{\vec{1}}}

% Nice plotting macro
\newcommand{\widgraph}[2]{\includegraphics[keepaspectratio,width=#1]{#2}}
%----------------------------------------end of macros-------------------


